Characterization of the Hamamatsu VUV4 MPPCs for nEXO

In this paper we report on the characterization of the Hamamatsu VUV4 (S/N: S13370-6152) Vacuum Ultra-Violet (VUV) sensitive Silicon Photo-Multipliers (SiPMs) as part of the development of a solution for the detection of liquid xenon scintillation light for the nEXO experiment. Various SiPM features, such as: dark noise, gain, correlated avalanches, direct crosstalk and Photon Detection Efficiency (PDE) were measured in a dedicated setup at TRIUMF. SiPMs were characterized in the range $163 \text{ } \text{K} \leq \text{T}\leq 233 \text{ } \text{K}$. At an over voltage of $3.1\pm0.2$ V and at $\text{T}=163 \text{ }\text{K}$ we report a number of Correlated Avalanches (CAs) per pulse in the $1 \upmu\text{s}$ interval following the trigger pulse of $0.161\pm0.005$. At the same settings the Dark-Noise (DN) rate is $0.137\pm0.002 \text{ Hz/mm}^{2}$. Both the number of CAs and the DN rate are within nEXO specifications. The PDE of the Hamamatsu VUV4 was measured for two different devices at $\text{T}=233 \text{ }\text{K}$ for a mean wavelength of $189\pm7\text{ nm}$. At $3.6\pm0.2$ V and $3.5\pm0.2$ V of over voltage we report a PDE of $13.4\pm2.6\text{ }\%$ and $11\pm2\%$, corresponding to a saturation PDE of $14.8\pm2.8\text{ }\%$ and $12.2\pm2.3\%$, respectively. Both values are well below the $24\text{ }\%$ saturation PDE advertised by Hamamatsu. More generally, the second device tested at $3.5\pm0.2$ V of over voltage is below the nEXO PDE requirement. The first one instead yields a PDE that is marginally close to meeting the nEXO specifications. This suggests that with modest improvements the Hamamatsu VUV4 MPPCs could be considered as an alternative to the FBK-LF SiPMs for the final design of the nEXO detector.

==> authors_full.tex <==
\newcommand{\Stanford}{1}
\newcommand{\Erlangen}{2}
\newcommand{\Yale}{3}
\newcommand{\Bama}{4}
\newcommand{\Triumph}{5}
\newcommand{\Carleton}{6}
\newcommand{\Indiana}{7}
\newcommand{\PNL}{8}
\newcommand{\Duke}{9}
\newcommand{\Illinois}{10}
\newcommand{\ITEP}{11}
\newcommand{\Sherbrooke}{13}
\newcommand{\SD}{12}
\newcommand{\LLNL}{14}
\newcommand{\RPI}{15}
\newcommand{\McGill}{16}
\newcommand{\IHEP}{17}
\newcommand{\IME}{18}
\newcommand{\Colorado}{19}
\newcommand{\BNL}{20}
\newcommand{\Laurentian}{21}
\newcommand{\Wilmington}{22}
\newcommand{\SLAC}{23}
\newcommand{\Drexel}{24}
\newcommand{\ORNL}{25}
\newcommand{\UMass}{26}
\newcommand{\Stony}{27}
\newcommand{\IBS}{28}
\newcommand{\LHEP}{29}


\author[\Stanford,\Erlangen,\Yale]{A.~Jamil\IEEEauthorrefmark{1}\thanks{\IEEEauthorrefmark{1}Corresponding Author}}%
\author[\Erlangen]{T.~Ziegler}%
\author[\Erlangen]{P.~Hufschmidt}%
\author[\Stanford]{G.~Li}%
\author[\Stanford]{L.~Lupin-Jimenez}%
\author[\Erlangen]{T.~Michel}%
\author[\Bama]{I.~Ostrovskiy}%
\author[\Triumph]{F.~Reti\`ere}%
\author[\Erlangen]{J.~Schneider}%
\author[\Erlangen]{M.~Wagenpfeil}%
\author[\Carleton]{A.~Alamre}%
\author[\Indiana]{J.~B.~Albert}%
\author[\Erlangen]{G.~Anton}%
\author[\PNL]{I.~J.~Arnquist}%
\author[\Carleton]{I.~Badhrees\IEEEauthorrefmark{2}\thanks{\IEEEauthorrefmark{2}Home institute King Abdulaziz City for Science and Technology,\\ ${}$\hspace{20pt} KACST, Riyadh 11442, Saudi Arabia}}%
\author[\Duke]{P.~S.~Barbeau}%
\author[\Illinois]{D.~Beck}%
\author[\ITEP]{V.~Belov}%
\author[\SD]{T.~Bhatta}%
\author[\Sherbrooke]{F.~Bourque}%
\author[\LLNL]{J.~P.~Brodsky}%
\author[\RPI]{E.~Brown}%
\author[\McGill,\Triumph]{T.~Brunner}%
\author[\ITEP]{A.~Burenkov}%
\author[\IHEP]{G.~F.~Cao\IEEEauthorrefmark{3}\thanks{\IEEEauthorrefmark{3}also at University of Chinese Academy of Sciences, \\ ${}$\hspace{22pt}Beijing 100049, China}}%
\author[\IME]{L.~Cao}%
\author[\IHEP]{W.~R.~Cen}%
\author[\Colorado]{C.~Chambers}%
\author[\Sherbrooke]{S.~A.~Charlebois}%
\author[\BNL]{M.~Chiu}%
\author[\Laurentian]{B.~Cleveland\IEEEauthorrefmark{4}\thanks{\IEEEauthorrefmark{4}also at SNOLAB, Ontario, Canada}}%
\author[\Illinois]{M.~Coon}%
\author[\Sherbrooke]{M.~C{\^o}t{\'e}}%
\author[\Colorado]{A.~Craycraft}%
\author[\Carleton]{W.~Cree}%
\author[\Stanford]{J.~Dalmasson}%
\author[\Wilmington]{T.~Daniels}%
\author[\McGill]{L.~Darroch}%
\author[\Indiana]{S.~J.~Daugherty}%
\author[\SD]{J.~Daughhetee}%
\author[\SLAC]{S.~Delaquis\IEEEauthorrefmark{5}\thanks{\IEEEauthorrefmark{5}deceased}}%
\author[\Laurentian]{A.~Der~Mesrobian-Kabakian}%
\author[\Stanford]{R.~DeVoe}%
\author[\Triumph]{J.~Dilling}%
\author[\IHEP]{Y.~Y.~Ding}%
\author[\Drexel]{M.~J.~Dolinski}%
\author[\SLAC]{A.~Dragone}%
\author[\Illinois]{J.~Echevers}%
\author[\ORNL]{L.~Fabris}%
\author[\Colorado]{D.~Fairbank}%
\author[\Colorado]{W.~Fairbank}%
\author[\Laurentian]{J.~Farine}%
\author[\UMass]{S.~Feyzbakhsh}%
\author[\Sherbrooke]{R.~Fontaine}%
\author[\Stanford]{D.~Fudenberg}%
\author[\Triumph]{G.~Gallina}%
\author[\BNL]{G.~Giacomini}%
\author[\Carleton,\Triumph]{R.~Gornea}%
\author[\Stanford]{G.~Gratta}%
\author[\Drexel]{E.~V.~Hansen}%
\author[\Colorado]{D.~Harris}%
\author[\SD]{M.~Hasan}%
\author[\LLNL]{M.~Heffner}%
\author[\Erlangen]{J.~H{\"o}{\ss}l}%
\author[\PNL]{E.~W.~Hoppe}%
\author[\LLNL]{A.~House}%
\author[\Bama]{M.~Hughes}%
\author[\McGill]{Y.~Ito}%
\author[\Colorado]{A.~Iverson}%
\author[\Carleton]{C.~Jessiman}%
\author[\Stanford]{M.~J.~Jewell}%
\author[\IHEP]{X.~S.~Jiang}%
\author[\ITEP]{A.~Karelin}%
\author[\Indiana,\SLAC]{L.~J.~Kaufman}%
\author[\Carleton]{T.~Koffas}%
\author[\Stanford]{S.~Kravitz\IEEEauthorrefmark{6}\thanks{\IEEEauthorrefmark{6}now at Lawrence Berkeley National Lab}}%
\author[\Triumph]{R.~Kr\"ucken}%
\author[\ITEP]{A.~Kuchenkov}%
\author[\Stony]{K.~S.~Kumar}%
\author[\Triumph]{Y.~Lan}%
\author[\SD]{A.~Larson}%
\author[\IBS]{D.~S.~Leonard}%
\author[\Illinois]{S.~Li}%
\author[\Yale]{Z.~Li}%
\author[\Laurentian]{C.~Licciardi}%
\author[\Drexel]{Y.~H.~Lin}%
\author[\IHEP]{P.~Lv}%
\author[\SD]{R.~MacLellan}%
\author[\SLAC]{B.~Mong}%
\author[\Yale]{D.~C.~Moore}%
\author[\McGill]{K.~Murray}%
\author[\ORNL]{R.~J.~Newby}%
\author[\IHEP]{Z.~Ning}%
\author[\Stony]{O.~Njoya}%
\author[\Sherbrooke]{F.~Nolet}%
\author[\Bama]{O.~Nusair}%
\author[\RPI]{K.~Odgers}%
\author[\SLAC]{A.~Odian}%
\author[\SLAC]{M.~Oriunno}%
\author[\PNL]{J.~L.~Orrell}%
\author[\PNL]{G.~S.~Ortega}%
\author[\PNL]{C.~T.~Overman}%
\author[\Sherbrooke]{S.~Parent}%
\author[\Bama]{A.~Piepke}%
\author[\UMass]{A.~Pocar}%
\author[\Sherbrooke]{J.-F.~Pratte}%
\author[\IME]{D.~Qiu}%
\author[\BNL]{V.~Radeka}%
\author[\BNL]{E.~Raguzin}%
\author[\BNL]{T.~Rao}%
\author[\BNL]{S.~Rescia}%
\author[\Laurentian]{A.~Robinson}%
\author[\Sherbrooke]{T.~Rossignol}%
\author[\SLAC]{P.~C.~Rowson}%
\author[\Sherbrooke]{N.~Roy}%
\author[\PNL]{R.~Saldanha}%
\author[\LLNL]{S.~Sangiorgio}%
\author[\Erlangen]{S.~Schmidt}%
\author[\Stanford]{A.~Schubert\IEEEauthorrefmark{7}\thanks{\IEEEauthorrefmark{7}now at OneBridge Solutions, Boise, ID}}
\author[\Carleton]{D.~Sinclair}%
\author[\SLAC]{K.~Skarpaas VIII}%
\author[\Bama]{A.~K.~Soma}%
\author[\Sherbrooke]{G.~St-Hilaire}%
\author[\ITEP]{V.~Stekhanov}%
\author[\LLNL]{T.~Stiegler}%
\author[\IHEP]{X.~L.~Sun}%
\author[\Stony]{M.~Tarka\IEEEauthorrefmark{8}\thanks{\IEEEauthorrefmark{8}now at University of Massachusetts, Amherst}}%
\author[\Colorado]{J.~Todd}%
\author[\IHEP]{T.~Tolba}%
\author[\McGill]{T.~I.~Totev}%
\author[\PNL]{R.~Tsang}%
\author[\BNL]{T.~Tsang}%
\author[\Sherbrooke]{F.~Vachon}%
\author[\Carleton]{B.~Veenstra}%
\author[\Bama]{V.~Veeraraghavan}%
\author[\Indiana]{G.~Visser}%
\author[\LHEP]{J.-L.~Vuilleumier}%
\author[\IME]{Q.~Wang}%
\author[\Carleton]{J.~Watkins}%
\author[\Stanford]{M.~Weber}%
\author[\IHEP]{W.~Wei}%
\author[\IHEP]{L.~J.~Wen}%
\author[\Laurentian]{U.~Wichoski}%
\author[\Erlangen]{G.~Wrede}%
\author[\Stanford]{S.~X.~Wu}%
\author[\IHEP]{W.~H.~Wu}%
\author[\Yale]{Q.~Xia}%
\author[\Illinois]{L.~Yang}%
\author[\Drexel]{Y.-R.~Yen}%
\author[\ITEP]{O.~Zeldovich}%
\author[\IHEP]{X.~Zhang\IEEEauthorrefmark{9}\thanks{\IEEEauthorrefmark{9}now at Tsinghua University, Beijing, China}}%
\author[\IHEP]{J.~Zhao}%
\author[\IME]{Y.~Zhou}%


\affil[\Stanford]{Physics Department, Stanford University, Stanford, California 94305, USA}
\affil[\Erlangen]{Erlangen Centre for Astroparticle Physics (ECAP), Friedrich-Alexander University Erlangen-N\"urnberg, Erlangen 91058, Germany}
\affil[\Yale]{Department of Physics, Yale University, New Haven, CT 06511, USA}
\affil[\Bama]{Department of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA}
\affil[\Triumph]{TRIUMF, Vancouver, British Columbia V6T 2A3, Canada}
\affil[\Carleton]{Department of Physics, Carleton University, Ottawa, Ontario K1S 5B6, Canada}
\affil[\Indiana]{Department of Physics and CEEM, Indiana University, Bloomington, IN 47405, USA}
\affil[\PNL]{Pacific Northwest National Laboratory, Richland, WA 99352, USA}
\affil[\Duke]{Department of Physics, Duke University, and Triangle Universities Nuclear Laboratory (TUNL), Durham, NC 27708, USA}
\affil[\Illinois]{Physics Department, University of Illinois, Urbana-Champaign, IL 61801, USA}
\affil[\ITEP]{Institute for Theoretical and Experimental Physics named by A.~I.~Alikhanov of National Research Center "Kurchatov Institute", Moscow 117218, Russia}
\affil[\SD]{Department of Physics, University of South Dakota, Vermillion, SD 57069, USA}
\affil[\Sherbrooke]{Universit\'e de Sherbrooke, Sherbrooke, Qu{\'e}bec J1K 2R1, Canada}
\affil[\LLNL]{Lawrence Livermore National Laboratory, Livermore, CA 94550, USA}
\affil[\RPI]{Department of Physics, Applied Physics and Astronomy, Rensselaer Polytechnic Institute, Troy, NY 12180, USA}
\affil[\McGill]{Physics Department, McGill University, Montr{\'e}al, Qu{\'e}bec H3A 2T8, Canada}
\affil[\IHEP]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affil[\IME]{Institute of Microelectronics, Chinese Academy of Sciences, Beijing 100029, China}
\affil[\Colorado]{Physics Department, Colorado State University, Fort Collins, CO 80523, USA}
\affil[\BNL]{Brookhaven National Laboratory, Upton, NY 11973, USA}
\affil[\Laurentian]{Department of Physics, Laurentian University, Sudbury, Ontario P3E 2C6, Canada}
\affil[\Wilmington]{Department of Physics and Physical Oceanography, University of North Carolina at Wilmington, Wilmington, NC 28403, USA}
\affil[\SLAC]{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affil[\Drexel]{Department of Physics, Drexel University, Philadelphia, PA 19104, USA}
\affil[\ORNL]{Oak Ridge National Laboratory, Oak Ridge, TN 37831, USA}
\affil[\UMass]{Amherst Center for Fundamental Interactions and Physics Department, University of Massachusetts, Amherst, MA 01003, USA}
\affil[\Stony]{Department of Physics and Astronomy, Stony Brook University, SUNY, Stony Brook, NY 11794, USA}
\affil[\IBS]{IBS Center for Underground Physics, Daejeon 34126, Korea}
\affil[\LHEP]{LHEP, Albert Einstein Center, University of Bern, Bern CH-3012, Switzerland}










